Transmitting Data Through Reconfigurable Intelligent Surface: A Spatial Sigma-Delta Modulation Approach

Transmitting data using the phases on reconfigurable intelligent surfaces (RIS) is a promising solution for future energy-efficient communication systems. Recent work showed that a virtual phased massive multiuser multiple-input-multiple-out (MIMO) transmitter can be formed using only one active antenna and a large passive RIS. In this paper, we are interested in using such a system to perform MIMO downlink precoding. In this context, we may not be able to apply conventional MIMO precoding schemes, such as the simple zero-forcing (ZF) scheme, and we typically need to design the phase signals by solving optimization problems with constant modulus constraints or with discrete phase constraints, which pose challenges with high computational complexities. In this work, we propose an alternative approach based on Sigma-Delta ($\Sigma\Delta$) modulation, which is classically famous for its noise-shaping ability. Specifically, first-order $\Sigma\Delta$ modulation is applied in the spatial domain to handle phase quantization in generating constant envelope signals. Under some mild assumptions, the proposed phased $\Sigma\Delta$ modulator allows us to use the ZF scheme to synthesize the RIS reflection phases with negligible complexity. The proposed approach is empirically shown to achieve comparable bit error rate performance to the unquantized ZF scheme.

==> sym_macro.tex <==
%make sure to keep this for convenience later
\newcommand\bw{\ensuremath{{\bm w}}}
\newcommand\bW{\ensuremath{{\bm W}}}
\newcommand\cW{\ensuremath{\bm{\mathcal{W}}}}
\newcommand\bbw{\ensuremath{{\bar{\bm w}}}}
\newcommand\bq{\ensuremath{{\bm q}}}
\newcommand\bx{\ensuremath{{\bm x}}}
\newcommand\by{\ensuremath{{\bm y}}}
\newcommand\bG{\ensuremath{{\bm G}}}
\newcommand\bh{\ensuremath{{\bm h}}}
\newcommand\bH{\ensuremath{{\bm H}}}
\newcommand\cH{\ensuremath{\bm{\mathcal{H}}}}
\newcommand\bbh{\ensuremath{\bar{\bm h}}}
\newcommand\hbh{\ensuremath{\hat{\bm h}}}
\newcommand\be{\ensuremath{{\bm e}}}
\newcommand\bz{\ensuremath{{\bm z}}}
\newcommand\bR{\ensuremath{{\bm R}}}
\newcommand\bT{\ensuremath{{\bm T}}}
\newcommand\bX{\ensuremath{{\bm X}}}
\newcommand\bZ{\ensuremath{{\bm Z}}}
\newcommand\cZ{\ensuremath{\bm{\mathcal{Z}}}}
\newcommand\bC{\ensuremath{{\bm C}}}
\newcommand\bc{\ensuremath{{\bm c}}}
\newcommand\ba{\ensuremath{{\bm a}}}
\newcommand\bba{\ensuremath{\bar{\bm a}}}
\newcommand\bA{\ensuremath{{\bm A}}}
\newcommand\bbA{\ensuremath{\bar{\bm A}}}
\newcommand\bb{\ensuremath{{\bm b}}}
\newcommand\bg{\ensuremath{{\bm g}}}
\newcommand\bB{\ensuremath{{\bm B}}}
\newcommand\blam{\ensuremath{{\bm \lambda}}}
\newcommand\bmu{\ensuremath{{\bm \mu}}}
\newcommand\balp{\ensuremath{{\bm \alpha}}}
\newcommand\bXi{\ensuremath{{\bm \Xi}}}
\newcommand\bPi{\ensuremath{{\bm \Pi}}}
\newcommand\bbPi{\ensuremath{\bar{\bm \Pi}}}
\newcommand\bF{\ensuremath{{\bm F}}}
\newcommand\bbF{\ensuremath{\bar{\bm F}}}
\newcommand\bd{\ensuremath{{\bm d}}}
\newcommand\bD{\ensuremath{{\bm D}}}
\newcommand\bu{\ensuremath{{\bm u}}}
\newcommand\bv{\ensuremath{{\bm v}}}
\newcommand\bSig{\ensuremath{{\bm \Sigma}}}
\newcommand\beeta{\ensuremath{{\bm \eta}}}


\newcommand\bY{\ensuremath{{\bm Y}}}
\newcommand\bYh{\ensuremath{{\bm Y}_{\rm H}}}
\newcommand\bYm{\ensuremath{{\bm Y}_{\rm M}}}
\newcommand\bV{\ensuremath{{\bm V}}}
\newcommand\bU{\ensuremath{{\bm U}}}
\newcommand\bVh{\ensuremath{{\bm V}_{\rm H}}}
\newcommand\bVm{\ensuremath{{\bm V}_{\rm M}}}
\newcommand\bs{\ensuremath{{\bm s}}}
\newcommand\bS{\ensuremath{{\bm S}}}
\newcommand\bE{\ensuremath{{\bm E}}}

\newcommand{\Zbb}{\mathbb{Z}}
\newcommand{\Nbb}{\mathbb{N}}
\newcommand{\Rbb}{\mathbb{R}}
\newcommand{\Cbb}{\mathbb{C}}
\newcommand{\Hbb}{\mathbb{H}}
\newcommand{\Sbb}{\mathbb{S}}

\newcommand{\setQ}{\mathcal{Q}}
\newcommand{\setF}{\mathcal{F}}
\newcommand{\setB}{\mathcal{B}}
\newcommand{\setX}{\mathcal{X}}
\newcommand{\setR}{\mathcal{R}}
\newcommand{\setU}{\mathcal{U}}
\newcommand{\setV}{\mathcal{V}}
\newcommand{\setS}{\mathcal{S}}
\newcommand{\setC}{\mathcal{C}}
\newcommand{\setD}{\mathcal{D}}
\newcommand{\setM}{\mathcal{M}}
\newcommand{\setN}{\mathcal{N}}
\newcommand{\setK}{\mathcal{K}}
\newcommand{\setP}{\mathcal{P}}
\newcommand{\setT}{\mathcal{T}}
\newcommand{\setL}{\mathcal{L}}

\newcommand{\ind}{I}
\newcommand{\N}{\mathcal{N}}
\newcommand{\CN}{\mathcal{CN}}
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\jj}{\mathfrak{j}}
\newcommand{\dec}{\mathrm{dec}}
\newcommand{\Diag}{\mathrm{Diag}}

\newcommand\bQ{\ensuremath{{\bm Q}}}
\newcommand\bLam{\ensuremath{{\bm \Lambda}}}
\newcommand\br{\ensuremath{{\bm r}}}

\newcommand\Ree{\ensuremath{{\rm Re}}}
\newcommand\Imm{\ensuremath{{\rm Im}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\bzero}{{\bm 0}}
\newcommand{\bone}{{\bm 1}}
\newcommand{\bI}{{\bm I}}
\newcommand*{\LargerCdot}{\raisebox{-0.25ex}{\scalebox{1.2}{$\cdot$}}}
\newcommand\vvec{\ensuremath{{\rm vec}}}
\newcommand\conv{\ensuremath{{\rm conv  \,}}}
\newcommand\sgn{\ensuremath{{\rm sgn}}}

\newcommand\dRi{\ensuremath{{d_i^R}}}
\newcommand\dIi{\ensuremath{{d_i^I}}}
\newcommand\SEPR{\ensuremath{{{\sf SEP}^R_{i,t}}}}
\newcommand\SEPI{\ensuremath{{{\sf SEP}^I_{i,t}}}}
\newcommand\aRi{\ensuremath{{a_{i,t}^R}}}
\newcommand\aIi{\ensuremath{{a_{i,t}^I}}}
\newcommand\bRi{\ensuremath{{b_{i,t}^R}}}
\newcommand\bIi{\ensuremath{{b_{i,t}^I}}}
\newcommand\cRi{\ensuremath{{c_{i,t}^R}}}
\newcommand\cIi{\ensuremath{{c_{i,t}^I}}}
\newcommand{\setbarU}{\bar{\mathcal{U}}}

%make sure to keep this for convenience later
\newcommand{\vx}{\bm x}
\newcommand{\vxbar}{\bm {\overline x}}
\newcommand{\vy}{\bm y}
\newcommand{\vs}{\bm s}
\newcommand{\vv}{\bm v}
\newcommand{\vg}{\bm g}
\newcommand{\mH}{\bm H}
\newcommand{\va}{\bm a}
\newcommand{\mA}{\bm A}
\newcommand{\mG}{\bm G}




%\newcommand\bd{\ensuremath{{\rm bd}}}
%\newcommand\inte{\ensuremath{{\rm int}}}
%%---- vectors -----------------
%\newcommand{\vct}{\bm{t}}
%\newcommand{\vcx}{\bm{x}}
%%---- sets --------------------
%\newcommand{\setB}{\mathcal{B}}
%\newcommand{\setR}{\mathcal{R}}
%\newcommand{\setW}{\mathcal{W}}
%\newcommand{\Rbb}{\mathbb{R}}
%\newcommand{\MVES}{\mathsf{MVES}}%make sure to keep this for convenience later
\newcommand\bw{\ensuremath{{\bm w}}}
\newcommand\bW{\ensuremath{{\bm W}}}
\newcommand\cW{\ensuremath{\bm{\mathcal{W}}}}
\newcommand\bbw{\ensuremath{{\bar{\bm w}}}}
\newcommand\bq{\ensuremath{{\bm q}}}
\newcommand\bx{\ensuremath{{\bm x}}}
\newcommand\by{\ensuremath{{\bm y}}}
\newcommand\bG{\ensuremath{{\bm G}}}
\newcommand\bh{\ensuremath{{\bm h}}}
\newcommand\bH{\ensuremath{{\bm H}}}
\newcommand\cH{\ensuremath{\bm{\mathcal{H}}}}
\newcommand\bbh{\ensuremath{\bar{\bm h}}}
\newcommand\hbh{\ensuremath{\hat{\bm h}}}
\newcommand\be{\ensuremath{{\bm e}}}
\newcommand\bz{\ensuremath{{\bm z}}}
\newcommand\bR{\ensuremath{{\bm R}}}
\newcommand\bT{\ensuremath{{\bm T}}}
\newcommand\bX{\ensuremath{{\bm X}}}
\newcommand\bZ{\ensuremath{{\bm Z}}}
\newcommand\cZ{\ensuremath{\bm{\mathcal{Z}}}}
\newcommand\bC{\ensuremath{{\bm C}}}
\newcommand\bc{\ensuremath{{\bm c}}}
\newcommand\ba{\ensuremath{{\bm a}}}
\newcommand\bba{\ensuremath{\bar{\bm a}}}
\newcommand\bA{\ensuremath{{\bm A}}}
\newcommand\bbA{\ensuremath{\bar{\bm A}}}
\newcommand\bb{\ensuremath{{\bm b}}}
\newcommand\bg{\ensuremath{{\bm g}}}
\newcommand\bB{\ensuremath{{\bm B}}}
\newcommand\blam{\ensuremath{{\bm \lambda}}}
\newcommand\bmu{\ensuremath{{\bm \mu}}}
\newcommand\balp{\ensuremath{{\bm \alpha}}}
\newcommand\bXi{\ensuremath{{\bm \Xi}}}
\newcommand\bPi{\ensuremath{{\bm \Pi}}}
\newcommand\bbPi{\ensuremath{\bar{\bm \Pi}}}
\newcommand\bF{\ensuremath{{\bm F}}}
\newcommand\bbF{\ensuremath{\bar{\bm F}}}
\newcommand\bd{\ensuremath{{\bm d}}}
\newcommand\bD{\ensuremath{{\bm D}}}
\newcommand\bu{\ensuremath{{\bm u}}}
\newcommand\bv{\ensuremath{{\bm v}}}
\newcommand\bSig{\ensuremath{{\bm \Sigma}}}
\newcommand\beeta{\ensuremath{{\bm \eta}}}


\newcommand\bY{\ensuremath{{\bm Y}}}
\newcommand\bYh{\ensuremath{{\bm Y}_{\rm H}}}
\newcommand\bYm{\ensuremath{{\bm Y}_{\rm M}}}
\newcommand\bV{\ensuremath{{\bm V}}}
\newcommand\bU{\ensuremath{{\bm U}}}
\newcommand\bVh{\ensuremath{{\bm V}_{\rm H}}}
\newcommand\bVm{\ensuremath{{\bm V}_{\rm M}}}
\newcommand\bs{\ensuremath{{\bm s}}}
\newcommand\bS{\ensuremath{{\bm S}}}
\newcommand\bE{\ensuremath{{\bm E}}}

\newcommand{\Zbb}{\mathbb{Z}}
\newcommand{\Nbb}{\mathbb{N}}
\newcommand{\Rbb}{\mathbb{R}}
\newcommand{\Cbb}{\mathbb{C}}
\newcommand{\Hbb}{\mathbb{H}}
\newcommand{\Sbb}{\mathbb{S}}

\newcommand{\setQ}{\mathcal{Q}}
\newcommand{\setF}{\mathcal{F}}
\newcommand{\setB}{\mathcal{B}}
\newcommand{\setX}{\mathcal{X}}
\newcommand{\setR}{\mathcal{R}}
\newcommand{\setU}{\mathcal{U}}
\newcommand{\setV}{\mathcal{V}}
\newcommand{\setS}{\mathcal{S}}
\newcommand{\setC}{\mathcal{C}}
\newcommand{\setD}{\mathcal{D}}
\newcommand{\setM}{\mathcal{M}}
\newcommand{\setN}{\mathcal{N}}
\newcommand{\setK}{\mathcal{K}}
\newcommand{\setP}{\mathcal{P}}
\newcommand{\setT}{\mathcal{T}}
\newcommand{\setL}{\mathcal{L}}

\newcommand{\ind}{I}
\newcommand{\N}{\mathcal{N}}
\newcommand{\CN}{\mathcal{CN}}
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\jj}{\mathfrak{j}}
\newcommand{\dec}{\mathrm{dec}}
\newcommand{\Diag}{\mathrm{Diag}}

\newcommand\bQ{\ensuremath{{\bm Q}}}
\newcommand\bLam{\ensuremath{{\bm \Lambda}}}
\newcommand\br{\ensuremath{{\bm r}}}

\newcommand\Ree{\ensuremath{{\rm Re}}}
\newcommand\Imm{\ensuremath{{\rm Im}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\bzero}{{\bm 0}}
\newcommand{\bone}{{\bm 1}}
\newcommand{\bI}{{\bm I}}
\newcommand*{\LargerCdot}{\raisebox{-0.25ex}{\scalebox{1.2}{$\cdot$}}}

%make sure to keep this for convenience later
\newcommand{\vx}{\bm x}
\newcommand{\vxbar}{\bm {\overline x}}
\newcommand{\vy}{\bm y}
\newcommand{\vs}{\bm s}
\newcommand{\vv}{\bm v}
\newcommand{\vg}{\bm g}
\newcommand{\mH}{\bm H}
\newcommand{\va}{\bm a}
\newcommand{\mA}{\bm A}
\newcommand{\mG}{\bm G}




%\newcommand\bd{\ensuremath{{\rm bd}}}
%\newcommand\inte{\ensuremath{{\rm int}}}
%%---- vectors -----------------
%\newcommand{\vct}{\bm{t}}
%\newcommand{\vcx}{\bm{x}}
%%---- sets --------------------
%\newcommand{\setB}{\mathcal{B}}
%\newcommand{\setR}{\mathcal{R}}
%\newcommand{\setW}{\mathcal{W}}
%\newcommand{\Rbb}{\mathbb{R}}
%\newcommand{\MVES}{\mathsf{MVES}}
